S-PLUS Clusters And Large-scale Environments (SCALE): I. A catalog of known clusters and groups in DR5 and a pilot study of Abell 4038

Within the framework of the Southern Photometric Local Universe Survey (S-PLUS), we introduce ${\bf S}$-PLUS ${\bf C}$lusters ${\bf A}$nd ${\bf L}$arge-scale ${\bf E}$nvironments (SCALE), a project dedicated to the study of galaxy clusters, groups, and their environments using 12-band photometry of S-PLUS combined with spectroscopic and photometric data from the literature. In this first paper, we present a catalog of 83 previously known systems in the redshift range $0.008 \leq z_{\rm spec} \leq 0.1$, for which we derive $R_{200}$, $M_{200}$, and velocity dispersions. Spectroscopic members are selected and matched with S-PLUS photometric redshifts (photo-$z$s). We find very good agreement between literature spectroscopic redshifts (spec-$z$s) and S-PLUS photometric redshifts (photo-$z$s), demonstrating the potential of the latter for cluster and group membership determination. As a proof of concept, we obtain photometric memberships for Abell 4038 using the Reliable Photometric Membership technique. A two- and three-dimensional analysis of the region within $10 h^{-1}$ Mpc ($10\times R_{200}$) from the center of Abell 4038 reveals about a dozen substructures including two additional clusters within $1.3\times R_{200}$ (Abell 4038B and Abell 4049). A color-luminosity segregation analysis shows that more luminous (less luminous) galaxies are redder (bluer), as expected. Low-concentration galaxies ($C \leq 2.5$) exhibit a weaker color-luminosity dependence, compared to higher-concentration ones, indicating mass-dependent evolutionary pathways that challenge a simple morphology-color dichotomy, with low-luminosity galaxies presenting bluer colors largely independent of concentration. The SCALE catalog provides a valuable basis for future studies of large-scale structures and their connection to galaxy evolution.

==> Supplementary_Tables.tex <==
\appendix

\section{Supplementary tables} \label{sec:sup-tables}


This section presents Tables 2a and 2b, the supplementary tables referenced in this work. Table \ref{tab:column_description} describes the columns used in Table \ref{tab:compilation}, which lists the spectroscopic members and interlopers for all clusters in Table \ref{tab:59clusters}, as defined in Section \ref{sec:Sample}. 


\begin{center}
\startlongtable
\begin{deluxetable*}{rp{0.75\linewidth}}
\tablecaption{%
Description of the columns in Table \ref{tab:compilation}, \ref{tab:a168}, listed in their order of appearance. Column names marked with an asterisk (*) denote patterns representing multiple columns. Table \ref{tab:compilation} includes an additional leading column with the cluster ID, while Table \ref{tab:a168} includes an extra column, flag_member_phot, indicating photometric membership status (0 = member; 1 = interloper; –1 = not considered; see Section \ref{sec:Elismar-Section}).
\label{tab:column_description}
}
%
\tablehead{%
\colhead{Column name} & \colhead{Description}
}
\startdata
*RA and Dec & right ascension and declination, epoch 2000, in degrees, 2 columns {\bf from here on - from S-PLUS DR5)}\\
PROB\_GAL & Probability of the object of being a galaxy, according to Nakazono et al. (XX)\\
*A and B & profile RMS along the major and minor axis, in degrees (2 columns) \\
THETA & position angle (CCW/World-x), in degrees\\
ELLIPTICITY & A\_IMAGE/B\_IMAGE\\
PETRO\_RADIUS & petrosian apertures in units of A or B\\
*FLUX\_RADIUS\_20/50/90 & radius enclosing 20\%, 50\% or 90\% of the total flux (3 columns) \\
*MU\_MAX\_\texttt{BAND} &  instrumental Peak surface brightness above background in \texttt{BAND}, where \texttt{BAND} is one of: g, r; e.g. MU\_MAX\_g (2 columns) \\
*BACKGROUND\_\texttt{BAND} & instrumental background at centroid position in  \texttt{BAND}, where \texttt{BAND} is one of: g, r; e.g. BACKGROUND\_r (2 columns) \\
*s2n\_\texttt{BAND}\_auto & signal to noise ratio of \texttt{BAND} measurement, where \texttt{BAND} is one of: g, r; e.g. s2n\_g\_auto (2 columns) \\
*\texttt{BAND}\_\texttt{APER} & S-PLUS DR5 AB-calibrated magnitude for the  \texttt{BAND} with aperture \texttt{APER}, where \texttt{BAND} is one of: J0378, J0395, J0410, J0430, J0515, J0660, J0861, g, i, r, u, z, and \texttt{APER} is one of: auto and PStotal; e.g. J0861\_PStotal. (24 columns) \\
*e\_\texttt{BAND}\_\texttt{APER} & S-PLUS DR5 magnitude error for the  \texttt{BAND} with aperture \texttt{APER}, where \texttt{BAND} is one of: J0378, J0395, J0410, J0430, J0515, J0660, J0861, g, i, r, u, z, and \texttt{APER} is one of: auto, PStotal, aper6; e.g. e\_r\_auto. (36 columns) \\
*\texttt{BAND}\_\texttt{APER} & extra S-PLUS DR5 AB-calibrated magnitude for the  \texttt{BAND} with aperture \texttt{APER}, where \texttt{BAND} is one of: g, r and \texttt{APER} is one of: aper3, aper6, res, iso, petro; e.g. r\_petro (10 columns) \\
zml & the single-point estimate of the photometric redshift\\
odds & area of the PDF contained within an interval of 0.02 of the PDF peak\\
*pdf\_weights\_\texttt{i} & weights of the gaussian components of the PDF mixture of the photometric redshift, where \texttt{i} is one of: 0, 1, 2; e.g. pdf\_weights\_0 (3 columns) \\
*pdf\_means\_\texttt{i} & means of the gaussian components of the PDF mixture of the photometric redshift, where \texttt{i} is one of: 0, 1, 2; e.g. pdf\_stds\_1 (3 columns) \\
*pdf\_stds\_\texttt{i} & standard deviations of the gaussian components of the PDF mixture of the photometric redshift, where \texttt{i} is one of: 0, 1, 2; e.g. pdf\_means\_2 (3 columns) \\
radius\_deg & distance to the cluster center, in degrees {\bf (from here on - derived in this work)}\\
radius\_Mpc & distance to the cluster center, in Mpc\\
flag\_member & indication if the object is an spectroscopic member or not of the cluster/group. 0 = member; 1 = interloper; -1 = not considered, following Section \ref{sec:Sample} \\
v & velocity, in km/s\\
v\_err & velocity error, in km/s\\
v\_offset & relative to the cluster central velocity, in km/s\\
z & spectroscopic redshift {\bf (from here on - taken from the compilation of Lima et al. 2025)} \\
e\_z & error in the spectroscopic redshift\\
f\_z & flag for the spectroscopic redshift quality\\
class\_spec & spectroscopic classification of the object\\
original\_class\_spec & original spectroscopic classification of the object (before grouping)\\
source & catalogue from which the the spectroscopic redshift was obtained\\
*mag\_\texttt{BAND} & Legacy Survey DR10 magnitude for band \texttt{BAND}, where \texttt{BAND} is one of: g, r, i, z, w1, w2, w3, w4; e.g: mag\_r (8 columns, {\bf from here on - taken from Tractor table of the Legacy Survey}) \\
type & Legacy Survey DR10 morphological classification, \\
shape\_r & Legacy Survey DR10 effective radius - radius that contains 50\% of the light, in arcsec, see more information in \url{https://www.legacysurvey.org/dr10/description/#morphological-classification}\\
\enddata
\end{deluxetable*}
\end{center}

% RC - Here we include the section 3.3 which was removed from the main body of the paper, with the description of the tables and interlopers in the 58 clusters/groups and the additional data for Abell 168 and MKW4. Cleaning all previous comments.

\subsection{Members and interlopers in 83 cluster/groups} 
\label{sec:membership-tables}

This section describes Table \ref{tab:compilation}. Its columns are detailed in Table \ref{tab:column_description} (see Section \ref{sec:sup-tables}), with two additions: (1) cluster$\_$name, included at the beginning of Table \ref{tab:compilation} to identify the host cluster/group, and (2) flag$\_$member$\_$photoz, appended to Tables \ref{tab:a168} and \ref{tab:mkw4} to indicate photometric membership, as defined in Section \ref{sec:Elismar-Section}.

Table \ref{tab:compilation} lists spec-z’s from the compilation of \citet{Lima+24}, photo-z’s from S-PLUS DR5, and additional parameters for galaxies within $5 \times R_{200}$ of the 83 clusters/groups, classified as spectroscopic members or interlopers using the shifting-gapper technique (Section \ref{sec:Sample}).

\begin{center}
\startlongtable
\tabletypesize{\small} % Reduz tamanho da fonte
\setlength{\tabcolsep}{2.5pt} % Reduz espaçamento entre colunas
\begin{deluxetable*}{*{15}{c}}
\tablecaption{
Spectroscopic members and interlopers for 83 clusters and groups\label{tab:compilation}
}
\tablehead{\colhead{Cluster ID} &
\colhead{RA} & \colhead{Dec} & \colhead{$\cdots$} & \colhead{r\_aper} & \colhead{g\_aper} & \colhead{$\cdots$} & \colhead{zml} & \colhead{odds} & \colhead{$\cdots$} & \colhead{v} & \colhead{v\_err} & \colhead{radius\_deg} & \colhead{radius\_Mpc} & \colhead{v\_offset}
}

\startdata
MKW4 & 180.975 &  1.891  & $\cdots$ & ------  & ------  & $\cdots$ &  ------ & ------  & $\cdots$ & 7325.729  & 3.297 & 0.014 & 0.021 & 1303.803  \\
MKW4 & 181.024 &  1.846  & $\cdots$ & 14.932  & 15.796  & $\cdots$ & 0.023   & 0.999  & $\cdots$ & 4909.101  & 2.098 & 0.053 & 0.079 & -1065.439   \\
MKW4 & 180.966 &  1.836  & $\cdots$ & ------  & ------  & $\cdots$ & ------  & ------ & $\cdots$ & 5686.763  & 9.293 & 0.057 & 0.084 & -303.026   \\
$\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$\\
\enddata
\tablecomments{The complete table is available in machine-readable form in the online journal; a portion is shown here for guidance on format and content. Owing to its wide format, only the most relevant columns are displayed (see Table \ref{tab:column_description}).}
\end{deluxetable*}
\end{center}





==> table1_backup.tex <==
\startlongtable
\begin{deluxetable*}{llllcccrrc}

\tablecaption{General properties of the 83 S-PLUS clusters and groups in the sample presented in this work, ordered by increasing spectroscopic redshift, from $z = 0.008$ to $0.1$. The coordinates (J2000) are in degrees. $N_\mathrm{Tot}$ is the total number of cluster members, selected as described in Section \ref{sec:Sample}, including those beyond the cluster virial radius (inside $10\ h^{-1}$ Mpc). $N_{200}$ is the number of cluster members within a radius of $R_{200}$, and off$_{M}$ gives the redshift offset described in Section \ref{sec:photo-z-spec-z-comparison}.}

\label{tab:59clusters}

\tablehead{
\colhead{Cluster/Group} & 
\colhead{R.A.} & 
\colhead{Dec.} & 
\colhead{$z$} & 
\colhead{$\sigma_{cl}$} & 
\colhead{$R_{200}$} & 
\colhead{$M_{200}$} & 
\colhead{$N_\mathrm{Tot}$} &
\colhead{$N_{200}$} & 
\colhead{$s$} \\
%
\colhead{} & 
\colhead{(deg)} & 
\colhead{(deg)} & 
\colhead{} & 
\colhead{(km s$^{-1}$)} & 
\colhead{($h^{-1}$ Mpc)} & 
\colhead{$(10^{14} M_{\odot})$} & 
\colhead{} &
\colhead{} & 
\colhead{}
}

\startdata
NGC3054           & 148.619110  & -25.70344  & 0.0077 &  
% 232.832  & 0.443218 & 0.099877  & 134  & 3   & ---- \\
 233  & 0.443 & 0.010  & 134  & 3   & --- \\
Antlia            & 157.505626 & -35.34220   & 0.009107 & 
%646.109  & 1.330019 & 2.702353  & 269  & 68  &  0.0027 \\
646  & 1.330 & 2.702  & 269  & 68  &  0.0027 \\
NGC3250           & 156.741641 & -39.90683 & 0.009213 & 
%116.48   & 0.254497 & 0.018935  & 168  & 5   &  0.0095 \\
116   & 0.254 & 0.019 & 168  & 5   &  0.0095 \\
NGC5044           & 198.849880  & -16.38553  & 0.0093   & 
%319.772  & 0.694731 & 0.385207  & 106  & 34  & 0.0059 \\
320  & 0.695 & 0.385  & 106  & 34  & 0.0059 \\
NGC3258           & 157.358909 & -35.497493 & 0.009307 & 
%640.73   & 1.319658 & 2.640165  & 262  & 67  & 0.0028 \\
641  & 1.320 & 2.640  & 262  & 67  & 0.0028 \\
NGC3263/NGC3256   & 157.277303 & -44.173905 & 0.009557 & 
%145.97   & 0.322283 & 0.038464  & 7    & 7   &  --- \\
146   & 0.322 & 0.038 &  7    & 7   &  --- \\
NGC3347           & 160.551132 & -36.379851 & 0.00975  & 
%168.501  & 0.367523 & 0.057053  & 121  & 7   &  0.0025 \\
168  & 0.367 & 0.057  & 121  & 7   &  0.0025 \\
NGC3091           & 150.094578 & -19.636829 & 0.012261 & 
%263.961  & 0.57534  & 0.219376  & 216  & 17  &  0.0017 \\
264  & 0.575  & 0.219  & 216  & 17  &  0.0017 \\
Hydra             & 159.196746 & -27.517746 & 0.012635 & 
%686.744  & 1.409045 & 3.22358   & 533  & 265 &  0.0022 \\
687  & 1.409 & 3.223   & 533  & 265 &  0.0022 \\
A194              & 21.42      & -1.40722   & 0.018    & 
%460.686  & 0.974335 & 1.071076  & 1382 & 151 & 0.0021 \\
461  & 0.974 & 1.071  & 1382 & 151 & 0.0021 \\
MKW4              & 180.99054  & 1.88829    & 0.02     & 
%536.428  & 1.118862 & 1.624886  & 1001 & 140 & 0.0047 \\
536  & 1.119 & 1.625  & 1001 & 140 & 0.0047 \\
A639              & 160.054114 & -46.269091 & 0.02061  & 
%465.072  & 0.975965 & 1.079044  & 46   & 42  &  0.0023 \\
465  & 0.976 & 1.079  & 46   & 42  &  0.0023 \\
MKW1              & 150.1337   & -2.9573    & 0.021    & 
%356.201  & 0.765779 & 0.521439  & 630  & 54  & 0.0034 \\
356  & 0.766 & 0.521  & 630  & 54  & 0.0034 \\
{[}YMV2007{]}7604 & 36.52796   & -0.33192   & 0.021311 & 
%135.687  & 0.296234 & 0.030194  & 211  & 6   &  --- \\
136  & 0.296 & 0.030  & 211  & 6   &  --- \\
HCG97             & 356.84558  & -2.32599   & 0.0218   & 
%460.496  & 0.962373 & 1.03572   & 28   & 28  & --- \\
460  & 0.962 & 1.036   & 28   & 28  & --- \\
WBL081            & 39.571697  & 2.082272   & 0.02192  & 
%447.375  & 0.945083 & 0.981002  & 670  & 81  & 0.0029 \\
447  & 0.945 & 0.981  & 670  & 81  & 0.0029 \\
IC1860            & 42.4038    & -31.1886   & 0.0223   & 
%438.39   & 0.923447 & 0.915479  & 151  & 40  & 0.0030 \\
438   & 0.923 & 0.915  & 151  & 40  & 0.0030 \\
A3581             & 211.887636 & -27.064399 & 0.022409 & 
%448.579  & 0.938288 & 0.960428  & 212  & 26  & 0.0033 \\
448  & 0.938 & 0.960  & 212  & 26  & 0.0033 \\
WBL074            & 37.911338  & 1.286248   & 0.022726 & 
%391.431  & 0.836071 & 0.679693  & 871  & 84  & 0.0032 \\
391  & 0.836 & 0.680  & 871  & 84  & 0.0032 \\
A2870             & 16.937456  & -46.924795 & 0.023216 & 
%273.218  & 0.594019 & 0.243882  & 112  & 22  & 0.0026\\
273  & 0.594 & 0.244  & 112  & 22  & 0.0026\\
NGC1132           & 43.236044  & -1.236168  & 0.023348 & 
%221.247  & 0.486982 & 0.134391  & 394  & 17  & 0.0047 \\
221  & 0.487 & 0.134  & 394  & 17  & 0.0047 \\
A2877             & 17.474568  & -45.920728 & 0.023874 & 
%705.331  & 1.433975 & 3.432954  & 227  & 105 & 0.0018 \\
705  & 1.434 & 3.433  & 227  & 105 & 0.0018 \\
A3389             & 95.535893  & -64.956146 & 0.026615 & 
%524.294  & 1.08189  & 1.478062  & 35   & 29  & --- \\
524  & 1.082  & 1.478  & 35   & 29  & --- \\
MKW8              & 220.15916  & 3.47639    & 0.027    & 
%521.646  & 1.08744  & 1.501461  & 1882 & 165 & 0.0010 \\
522  & 1.087  & 1.501  & 1882 & 165 & 0.0010 \\
{[}YMV2007{]}2116 & 46.385427  & -0.37856   & 0.027619 & 
%504.046  & 1.049948 & 1.352232  & 709  & 61  & 0.0008 \\
504  & 1.050 & 1.352  & 709  & 61  & 0.0008 \\
%\nodata           & \nodata  & \nodata  &\nodata & \nodata  &\nodata&\nodata & \nodata & \nodata & \nodata \\
A4049             & 357.946318 & -28.35915 & 0.028116 & 
%315.798  & 0.679298 & 0.366378  & 338  & 28  & 0.0013 \\
316  & 0.679 & 0.366  & 338  & 28  & 0.0013 \\
A4038             & 356.929990  & -28.14139  & 0.0282   & 
%741.624  & 1.498758 & 3.935283  & 574  & 114 & 0.0015 \\
742  & 1.499 & 3.935  & 566  & 112 & 0.0015 \\
A3744             & 316.80124  & -25.43806  & 0.0381   & 
%588.517  & 1.204806 & 2.063191  & 117  & 68  & 0.0034 \\
588  & 1.205 & 2.063  & 117  & 68  & 0.0034 \\
A3733             & 315.418321 & -28.042699 & 0.03898  & 
%593.082  & 1.213196 & 2.108332  & 96   & 72  & -0.0007 \\
593  & 1.213 & 2.108  & 96   & 72  & -0.0007 \\
WBL288            & 162.426979 & 0.337996   & 0.039426 & 
%322.235  & 0.691517 & 0.390603  & 851  & 43  &  -0.0011 \\
322  & 0.691 & 0.391  & 851  & 43  &  -0.0011 \\
CL1058+0137       & 164.56675  & 1.623722   & 0.039555 & 
%381.042  & 0.809703 & 0.627131  & 1233 & 94  & -0.0011 \\
381  & 0.810 & 0.627  & 1233 & 94  & -0.0011 \\
A463              & 67.307578  & -53.825798 & 0.040085 & 
%628.191  & 1.276409 & 2.457912  & 170  & 56  & 0.0021 \\
628  & 1.276 & 2.458  & 170  & 56  & 0.0021 \\
A957              & 153.414132 & -0.911491  & 0.044159 & 
%655.556  & 1.329625 & 2.788993  & 1719 & 152 & 0.0029 \\
655  & 1.330 & 2.789  & 1719 & 152 & 0.0029 \\
A119              & 14.07625   & -1.21667   & 0.0442   & 
%859.634  & 1.705662 & 5.887835  & 1099 & 278 & 0.0014 \\
860  & 1.706 & 5.888  & 1099 & 278 & 0.0014 \\
A168              & 18.744541  & 0.41168    & 0.044841 & 
%523.285  & 1.081385 & 1.501344  & 1135 & 155 & 0.0017 \\
523  & 1.081 & 1.501  & 1135 & 155 & 0.0017 \\
MS0116.3-0115     & 19.72339   & -1.00391   & 0.0452   & 
%438.85   & 0.91694  & 0.915607  & 866  & 57  & 0.0016 \\
439   & 0.917  & 0.916  & 866  & 57  & 0.0016 \\
A3716             & 312.880616 & -52.68798  & 0.045716 & 
%762.069  & 1.525785 & 4.220632  & 464  & 200 & --- \\
762  & 1.526 & 4.221  & 464  & 200 & --- \\
A1631             & 193.220092 & -15.420825 & 0.046422 & 
%652.71   & 1.323506 & 2.756545  & 639  & 195 &  0.0011 \\
653   & 1.323 & 2.756  & 639  & 195 &  0.0011 \\
{[}YMV2007{]}7609 & 17.09684   & 0.08978    & 0.04688  & 
%43.582   & 0.318703 & 0.001148  & 5    & 4   & 0.0005 \\
43   & 0.319 & 0.001  & 5    & 4   & 0.0005 \\
A1644             & 194.29042  & -17.40028  & 0.0473   & 
%808.024  & 1.608435 & 4.95174   & 654  & 185 & 0.0004 \\
808  & 1.608 & 4.952  & 654  & 185 & 0.0004 \\
MCXCJ1121.7+0249  & 170.424379 & 2.814099   & 0.048607 & 
%575.358  & 1.177068 & 1.943071  & 574  & 134 & --- \\
575  & 1.177 & 1.943  & 574  & 134 & --- \\
A4059             & 359.25958  & -34.76056  & 0.0487   & 
%791.396  & 1.577108 & 4.674193  & 454  & 189 & 0.0056 \\
791  & 1.577 & 4.674  & 454  & 189 & 0.0056 \\
A2717             & 0.80042    & -35.92722  & 0.049    & 
%576.326  & 1.176927 & 1.943095  & 426  & 83  & 0.0065 \\
576  & 1.177 & 1.943  & 426  & 83  & 0.0065 \\
IC1365            & 318.479955 & 2.569276   & 0.049264 & 
%662.074  & 1.338566 & 2.859386  & 849  & 156 & --- \\
662  & 1.338 & 2.859  & 849  & 156 & --- \\
MCXCJ0413.9-3805  & 63.502253  & -38.110323 & 0.049812 & 
%470.066  & 0.969191 & 1.085943  & 158  & 31  & --- \\
470  & 0.969 & 1.086  & 158  & 31  & --- \\
A620              & 147.25     & -26.0335   & 0.0499   & 
%544.173  & 1.024618 & 1.28322   & 5    & 5   & --- \\
544  & 1.025 & 1.283  & 5    & 5   & --- \\
{[}YMV2007{]}841  & 16.084398  & -0.239089  & 0.050225 & 
%247.695  & 0.529222 & 0.176873  & 85   & 13  & -0.0039 \\
248  & 0.529 & 0.177  & 85   & 13  & -0.0039 \\
RXJ2137.1+0026    & 324.27792  & 0.4475     & 0.051    & 
%316.272  & 0.671427 & 0.361464  & 358  & 24  & 0.0052 \\
316  & 0.671 & 0.361  & 358  & 24  & 0.0052 \\
{[}YMV2007{]}4713 & 214.3499   & 0.088181   & 0.052894 & 
%251.985  & 0.538199 & 0.1865    & 955  & 14  & 0.0015 \\
252  & 0.538 & 0.186   & 955  & 14  & 0.0015 \\
A151              & 17.20875   & -15.41     & 0.0533   & 
%716.363  & 1.436321 & 3.546264  & 489  & 177 & 0.0005 \\
716  & 1.436 & 3.546  & 489  & 177 & 0.0005 \\
MKW6              & 214.4027   & 2.06187    & 0.05367  & 
%588.586  & 1.199136 & 2.064312  & 1231 & 144 &  0.0025 \\
588  & 1.199 & 2.064  & 1231 & 144 &  0.0025 \\
A978              & 155.12047  & -6.511394  & 0.054137 & 
%595.694  & 1.211795 & 2.131325  & 897  & 128 & 0.0025 \\
596  & 1.212 & 2.131  & 897  & 128 & 0.0025 \\
A993              & 155.462316 & -4.928168  & 0.054516 & 
%400.31   & 0.839893 & 0.709888  & 832  & 66  & 0.0004 \\
400   & 0.840 & 0.710  & 832  & 66  & 0.0004 \\
A3225             & 62.37078   & -59.604333 & 0.054979 & 
%1050.793 & 2.028371 & 10.003511 & 50   & 49  &  0.0021 \\
1051 & 2.028 & 10.003 & 50   & 49  &  0.0021 \\
{[}YMV2007{]}49   & 214.33151  & 2.34428    & 0.05512  & 
%305.122  & 0.632561 & 0.303441  & 932  & 10  & 0.0012 \\
305  & 0.632 & 0.303  & 932  & 10  & 0.0012 \\
{[}YMV2007{]}514  & 24.315452  & -0.485475  & 0.055666 & 
%189.748  & 0.41609  & 0.086409  & 164  & 16  & -0.0001 \\
190  & 0.416  & 0.086  & 164  & 16  & -0.0001 \\
A133              & 15.67542   & -21.87361  & 0.0566   & 
%667.036  & 1.317141 & 2.74333   & 41   & 17  & 0.0015 \\
667  & 1.317 & 2.743   & 41   & 17  & 0.0015 \\
ESO351-021        & 13.7558    & -35.319479 & 0.056897 & 
%383.129  & 0.762836 & 0.533086  & 17   & 7   & -0.0028 \\
383  & 0.763 & 0.533  & 17   & 7   & -0.0028 \\
A2457             & 338.91998  & 1.48489    & 0.0578   & 
%684.791  & 1.375618 & 3.128757  & 1227 & 206 & 0.0005 \\
685  & 1.376 & 3.129  & 1227 & 206 & 0.0005 \\
A3880             & 336.971154 & -30.589133 & 0.057983 & 
%642.159  & 1.29534  & 2.612792  & 471  & 115 & -0.0039 \\
642  & 1.295  & 2.613  & 471  & 115 & -0.0039 \\
A2415             & 331.41876  & -5.59333   & 0.0581   & 
%684.335  & 1.373753 & 3.116943  & 761  & 146 & 0.0014 \\
684  & 1.374 & 3.117  & 761  & 146 & 0.0014 \\
A970              & 154.3475   & -10.6775   & 0.0587   & 
%777.293  & 1.543075 & 4.419899  & 179  & 138 & 0.0005 \\
777  & 1.543 & 4.420  & 179  & 138 & 0.0005 \\
A3158             & 55.739224  & -53.642113 & 0.059279 & 
%1024.507 & 1.988828 & 9.468539  & 342  & 298 & 0.0024 \\
1024 & 1.989 & 9.468  & 342  & 298 & 0.0024 \\
A3223             & 62.078512  & -30.902245 & 0.059778 & 
%589.614  & 1.193746 & 2.048494  & 181  & 60  &  0.0002 \\
590  & 1.194 & 2.048  & 181  & 60  &  0.0002 \\
A3266             & 67.842273  & -61.44816  & 0.059788 & 
%1275.547 & 2.430956 & 17.299525 & 536  & 428 & --- \\
1275 & 2.431 & 17.299 & 536  & 428 & --- \\
A3128             & 52.47917   & -52.56667  & 0.0599   & 
%825.962  & 1.632615 & 5.24084   & 815  & 381 & -0.0002 \\
826  & 1.633 & 5.241   & 815  & 381 & -0.0002 \\
CODEX-59603       & 359.419804 & 0.798581   & 0.061004 & 
%256.897  & 0.542878 & 0.192892  & 195  & 12  &  0.0 \\
257  & 0.543 & 0.193  & 195  & 12  &  0.0 \\
A3809             & 326.74084  & -43.91     & 0.0623   & 
%541.987  & 1.106775 & 1.636533  & 264  & 117 & -0.0022 \\
542  & 1.107 & 1.636  & 264  & 117 & -0.0022 \\
A2734             & 2.83625    & -28.855    & 0.0625   & 
%629.544  & 1.268386 & 2.463683  & 680  & 92  & -0.0011 \\
629  & 1.268 & 2.464  & 680  & 92  & -0.0011 \\
A3135             & 53.50935   & -39.00015  & 0.0642   & 
%719.021  & 1.426049 & 3.507054  & 190  & 46  & -0.0014 \\
719  & 1.426 & 3.507  & 190  & 46  & -0.0014 \\
A3122             & 50.57625   & -41.33889  & 0.0643   & 
%736.168  & 1.461581 & 3.776151  & 129  & 78  &  -0.0027 \\
736  & 1.461 & 3.776  & 129  & 78  &  -0.0027 \\
A1069             & 159.935    & -8.68361   & 0.065    & 
%684.891  & 1.369006 & 3.105196  & 478  & 103 & -0.0050 \\
685  & 1.369 & 3.105  & 478  & 103 & -0.0050 \\
MCXCJ0340-4542    & 55.192363  & -45.682315 & 0.068939 & 
%349.816  & 0.71511  & 0.444261  & 19   & 11  & 0.0037 \\
350  & 0.715  & 0.444  & 19   & 11  & 0.0037 \\
A3104             & 48.5825    & -45.42417  & 0.073    & 
%362.794  & 0.699061 & 0.416646  & 36   & 5   & -0.0042 \\
363  & 0.699 & 0.417  & 36   & 5   & -0.0042 \\
A3112             & 49.509398  & -44.251381 & 0.073973 & 
%398.65   & 0.820878 & 0.675255  & 59   & 24  &  -0.0044 \\
399   & 0.821 & 0.675  & 59   & 24  &  -0.0044 \\
MCXCJ0229.3-3332  & 37.337455  & -33.50317  & 0.076514 & 
%677.308  & 1.341868 & 2.956868  & 213  & 45  & -0.0036 \\
677  & 1.342 & 2.957  & 213  & 45  & -0.0036 \\
WHLJ012023-000444 & 20.09641   & -0.07898   & 0.078    & 
%360.448  & 0.746549 & 0.509922  & 337  & 23  &  0.0013 \\
360  & 0.746 & 0.509922  & 337  & 23  &  0.0013 \\
{[}YMV2007{]}3820 & 201.835649 & 1.276449   & 0.080432 & 
%498.156  & 1.011226 & 1.270287  & 901  & 47  & --- \\
498  & 1.011 & 1.270  & 901  & 47  & --- \\
MCXCJ1326.2+0013  & 201.5733   & 0.2251     & 0.0826   & 
%523.555  & 1.059026 & 1.462162  & 984  & 61  & 0.0048 \\
523  & 1.059 & 1.462  & 984  & 61  & 0.0048 \\
A1750             & 202.80154  & -1.71417   & 0.0837   & 
%366.724  & 0.759304 & 0.539497  & 565  & 30  & --- \\
367 & 0.759 & 0.539  & 565  & 30  & --- \\
{[}YMV2007{]}4832 & 149.976097 & -0.234508  & 0.090357 & 
%421.946  & 0.849138 & 0.759468  & 554  & 15  & 0.0001 \\
422  & 0.849 & 0.759  & 554  & 15  & 0.0001 \\
A2440             & 335.97043  & -1.63778   & 0.0906   & 
%811.126  & 1.579778 & 4.89178   & 479  & 135 & 0.0192 \\
811  & 1.580 & 4.892  & 479  & 135 & 0.0192 \\
{[}YMV2007{]}1540 & 154.94673  & -0.646272  & 0.093247 & 
%421.418  & 0.857986 & 0.785687  & 645  & 29  & 0.0168 \\
421  & 0.858 & 0.786  & 645  & 29  & 0.0168 \\
%\nodata           & \nodata  & \nodata  &\nodata & \nodata  &\nodata&\nodata & \nodata & \nodata & \nodata \\
A954              & 153.436363 & -0.121503  & 0.094641 & 
%746.393  & 1.459459 & 3.872417  & 1002 & 93  & -0.0024
746  & 1.459 & 3.872  & 1002 & 93  & -0.0024
\enddata
\tablecomments{The digital version of this table is available at \url{https://splus-scale.github.io/publications/1}}
\end{deluxetable*}
